Whale: Efficient Giant Model Training over Heterogeneous GPUs

The scaling up of deep neural networks has been demonstrated to be effective in improving model quality, but also encompasses several training challenges in terms of training efficiency, programmability, and resource adaptability. We present Whale, a general and efficient distributed training framework for giant models. To support various parallel strategies and their hybrids, Whale generalizes the programming interface by defining two new primitives in the form of model annotations, allowing for incorporating user hints. The Whale runtime utilizes those annotations and performs graph optimizations to transform a local deep learning DAG graph for distributed multi-GPU execution. Whale further introduces a novel hardware-aware parallel strategy, which improves the performance of model training on heterogeneous GPUs in a balanced manner. Deployed in a production cluster with 512 GPUs, Whale successfully trains an industry-scale multimodal model with over ten trillion model parameters, named M6, demonstrating great scalability and efficiency.

==> heto-algo.tex <==
% % \begin{algorithm}[t]
% % \caption{Keyword Oriented Search}	\label{algo:kos}
% % \SetKwProg{Function}{Function}{}{}

% % \Function{KOSearch ($ v_{st} $, $ W $)}
% % {	
% % 	$ rq\leftarrow \{SR.root\}, dq\leftarrow \{\{v_{st}\}\} $\\
% % 	Refine time for keyword tag involving TR\\
% % 	\While{$ rq \ne \emptyset $}
% % 	{
% % 		$  V \leftarrow dq.pop()$,
% % 		$ R_C \leftarrow rq.pop();$\\
% % 		\If{$ R_C $ is the relation to check}
% % 		{
% % 			$ W\leftarrow$ the set of keyword tags to check in $ R_C $ \\
% % 			\For{$ v\in V $}
% % 			{
% % 				\For{$ w \in W $}
% % 					{	\If{$ w.k $ is wild \textbf{or} $ w.k\in v.K $}{$ W\leftarrow W\setminus w $, \textbf{break}}
% % 					}
% % 					\If{$ W=\emptyset $}{\textbf{break}}
% % 			}
% % 			\If{$ W\ne \emptyset $}{\textbf{return false}}
% % 	}
% % 		\ForEach{$ NR \in R_C.neighbors $}
% % 		{
% % 			$ rq.add(NR); $
% % 			D $ \leftarrow \emptyset $\\
% % 			\ForEach{$ u\in V $}{
% % 						\If{$ NR $ has time constraint T}
% % 						{$ V_N\leftarrow$ u's neighbor nodes overlap T}
% % 						\Else{$ V_N\leftarrow$ u's neighbor nodes}
% % 						$ D\leftarrow D\bigcup V_N$
% % 				}			
% % 				$ dq.add(D) $
% % 		}
% % 	}
% % 	\textbf{return} true
% % }
% % \end{algorithm}

% \begin{algorithm}[t]
% \caption{Hardware-aware Data Parallel Partition}	\label{algo:heto-dp}
% \SetKwProg{Function}{Function}{}{}
% \Function{$DP\_Partition$ (graph, bs, GPUs)}
% {
%   $flop\_ratios \leftarrow [], mem\_ratios \leftarrow \{\}$ \\
%   $N \leftarrow len(GPUs)$ \\
%   $total\_flops \leftarrow \sum_{i=0}^{N}$ GPUs[i].flops \\
%   \ForEach{$ i \in range(N) $}
%   {
%     $bs_{i} \leftarrow bs * GPUs[i].flops / total\_flops $\label{heto-dp:line:set-bs} \\
%     %$mem_{i} \leftarrow profile\_mem(graph, bs_{i}) $ \\
%     $mem\_ratios.add(\frac{profile\_mem(graph, bs_{i})}{GPUs[i].mem}) $ \\
%     %$flop_i \leftarrow profile\_flop(graph, bs_{i}) $ \\
%     $flop\_ratios[i] \leftarrow (\frac{profile\_flop(graph, bs_{i})}{GPUs[i].flops}, i) $ \\
%   }
%   \While{$any(mem\_ratios > 1)$}
%   {
%     $j = argmax(mem\_ratios)$ \\
%     $bs_{j} \leftarrow bs_{j} - 1$ \\
%     $flop\_indices = sort(flop\_ratios.values())$ \\
%     $mem_j \leftarrow profile\_mem(stages[j], mbs) $ \\
%     \ForEach{$ \_, k \in flop\_indices $}
%     { 
%       $bs_{k} \leftarrow bs_{k} + 1$ \\
%       $mem_k \leftarrow profile\_mem(graph, bs_{k}) $ \\
%       \If{$mem_k > GPUs[k].mem$}{$bs_{k} \leftarrow bs_{k} - 1$\\ $flop\_ratios.remove(k)$}\\
%       \Else{$ mem\_ratios[k] \leftarrow \frac{mem_k}{GPUs[k].mem} \\mem\_ratios[j] \leftarrow \frac{mem_j}{GPUs[j].mem} $ \\
%       $flop_k \leftarrow profile\_flop(graph, bs_{k})$ \\
%       $flop\_ratios[k] \leftarrow (\frac{flop_k}{GPUs[k].flops}, k) $ \\$break$}
%     }
%   }
% }
% \end{algorithm}


% \begin{algorithm}[t]
% \caption{Hardware-aware Pipeline Stage Partition}	\label{algo:heto-pipeline}
% \SetKwProg{Function}{Function}{}{}
% \Function{$Pipeline\_Partition$ (graph, bs, GPUs)}
% {
%   $flop\_ratios \leftarrow [], mem\_ratios \leftarrow \{\}, weights \leftarrow [] $ \\
%   $ ops \leftarrow topo\_sort(graph.ops) $\\
%   $N \leftarrow len(GPUs)$ \\
%   $total\_flops \leftarrow \sum_{i=0}^{N}$ GPUs[i].flops \\
%   \ForEach{$ i \in range(N) $}
%   {
%     $ weights[i]  \leftarrow GPUs[i].flops / total\_flops $\\
%   }
% %  $avg\_flop  \leftarrow \sum_{i} ops[i].flop / N$ \\
%   $stages \leftarrow partition\_stages(ops, weights)$ \\
%   $mbs \leftarrow \min_{i=0}^{N}max\_micro\_bs(stage[i], GPUs[i]) $ \\
%   $mbs \leftarrow \max (mbs, 1) $ \\
%   \ForEach{$ i \in range(N) $}
%   {
%     %$mem_{i} \leftarrow profile\_mem(stages[i], mbs) $ \\
%     $mem\_ratios.add(\frac{profile\_mem(stages[i], mbs)}{GPUs[i].mem}) $ \\
%     %$flop_i \leftarrow profile\_flop(stages[i], mbs) $ \\
%     $flop\_ratios[i] \leftarrow (\frac{profile\_flop(stages[i], mbs)}{GPUs[i].flops}, i) $ \\
%  }
%   \While{$flop\_ratios \ne \emptyset \And any(mem\_ratios > 1)$}
%   {
%     $j = argmax(mem\_ratios)$ \\
%   % $flop\_ratios.pop(j)$ \\
%     $flop\_indices = sort(flop\_ratios.values())$ \\
%     $mem_j \leftarrow profile\_mem(stages[j], mbs) $ \\
%     \If{$mem_j \leq GPUs[j].mem$}{$flop\_ratios.pop(j)$}
%     \ForEach{$ \_, k \in flop\_indices $}
%     { 
%       $shift\_op(stages, j, k) $\\
%       $mem_k \leftarrow profile\_mem(stages[k], mbs) $ \\
%       \If{$mem_k > GPUs[k].mem$}{$shift\_op(stages, k, j) $\\ $flop\_ratios.remove(k)$}\\
%       \Else{$ mem\_ratios[k] \leftarrow \frac{mem_k}{GPUs[k].mem}  \\
%       mem\_ratios[j] \leftarrow \frac{mem_j}{GPUs[j].mem} $ \\
%       $ flop_k \leftarrow profile\_flop(stages[k], mbs) $ \\
%       $flop\_ratios[k] \leftarrow (\frac{flop_k}{GPUs[k].flops}, k) $ \\
%       $break$}
%     }
%   }
% }
% \end{algorithm}


% % \begin{algorithm}[t]
% % \caption{Keyword Oriented Search}	\label{algo:kos}
% % \SetKwProg{Function}{Function}{}{}

% % \Function{KOSearch ($ v_{st} $, $ W $)}
% % {	
% % 	$ rq\leftarrow \{SR.root\}, dq\leftarrow \{\{v_{st}\}\} $\\
% % 	Refine time for keyword tag involving TR\\
% % 	\While{$ rq \ne \emptyset $}
% % 	{
% % 		$  V \leftarrow dq.pop()$,
% % 		$ R_C \leftarrow rq.pop();$\\
% % 		\If{$ R_C $ is the relation to check}
% % 		{
% % 			$ W\leftarrow$ the set of keyword tags to check in $ R_C $ \\
% % 			\For{$ v\in V $}
% % 			{
% % 				\For{$ w \in W $}
% % 					{	\If{$ w.k $ is wild \textbf{or} $ w.k\in v.K $}{$ W\leftarrow W\setminus w $, \textbf{break}}
% % 					}
% % 					\If{$ W=\emptyset $}{\textbf{break}}
% % 			}
% % 			\If{$ W\ne \emptyset $}{\textbf{return false}}
% % 	}
% % 		\ForEach{$ NR \in R_C.neighbors $}
% % 		{
% % 			$ rq.add(NR); $
% % 			D $ \leftarrow \emptyset $\\
% % 			\ForEach{$ u\in V $}{
% % 						\If{$ NR $ has time constraint T}
% % 						{$ V_N\leftarrow$ u's neighbor nodes overlap T}
% % 						\Else{$ V_N\leftarrow$ u's neighbor nodes}
% % 						$ D\leftarrow D\bigcup V_N$
% % 				}			
% % 				$ dq.add(D) $
% % 		}
% % 	}
% % 	\textbf{return} true
% % }
% % \end{algorithm}

% \begin{algorithm}[t]
% \caption{Hardware-aware Data Parallel Partition}	\label{algo:heto-dp}
% \SetKwProg{Function}{Function}{}{}
% \Function{$DP\_Partition$ (replicas, global\_bs, GPUs)}
% {
%   $flop\_ratios \leftarrow [], mem\_ratios \leftarrow \{\}$ \\
%   $N \leftarrow len(GPUs)$ \\
%   $total\_flops \leftarrow \sum_{i=0}^{N}$ GPUs[i].flops \\
%   \ForEach{$ i \in range(N) $}
%   {
%     % $bs_{i} \leftarrow  \\
%     $ replicas[i].bs \leftarrow \frac{global\_bs * GPUs[i].flops}{total\_flops} $\label{heto-dp:line:set-bs}  \\
%     $mem\_ratios.add(\frac{profile\_mem(replicas[i])}{GPUs[i].mem}) $ \\
%     %$flop_i \leftarrow profile\_flop(graph, bs_{i}) $ \\
%     $flop\_ratios[i] \leftarrow (\frac{profile\_flop(replicas[i])}{GPUs[i].flops}, i) $ \\
%   }
%   \If{$any(mem\_ratios > 1$)}{$PSVF(replicas, flop\_ratios, mem\_ratios, GPUs, shift\_batch)$ \\}
% %   \While{$any(mem\_ratios > 1)$}
% %   {
% %     $j = argmax(mem\_ratios)$ \\
% %     $bs_{j} \leftarrow bs_{j} - 1$ \\
% %     $flop\_indices = sort(flop\_ratios.values())$ \\
% %     $mem_j \leftarrow profile\_mem(stages[j], mbs) $ \\
% %     \ForEach{$ \_, k \in flop\_indices $}
% %     { 
% %       $bs_{k} \leftarrow bs_{k} + 1$ \\
% %       $mem_k \leftarrow profile\_mem(graph, bs_{k}) $ \\
% %       \If{$mem_k > GPUs[k].mem$}{$bs_{k} \leftarrow bs_{k} - 1$\\ $flop\_ratios.remove(k)$}\\
% %       \Else{$ mem\_ratios[k] \leftarrow \frac{mem_k}{GPUs[k].mem} \\mem\_ratios[j] \leftarrow \frac{mem_j}{GPUs[j].mem} $ \\
% %       $flop_k \leftarrow profile\_flop(graph, bs_{k})$ \\
% %       $flop\_ratios[k] \leftarrow (\frac{flop_k}{GPUs[k].flops}, k) $ \\$break$}
% %     }
% %   }
% }
% \Function{$shift\_batch (replicas, i, j)$}
% {
%   $replicas[i].bs \leftarrow replicas[i].bs - 1$ \\
%   $replicas[j].bs \leftarrow replicas[j].bs + 1$ \\
% }
% \end{algorithm}




